One Fits All:Power General Time Series Analysis by Pretrained LM

Although we have witnessed great success of pre-trained models in natural language processing (NLP) and computer vision (CV), limited progress has been made for general time series analysis. Unlike NLP and CV where a unified model can be used to perform different tasks, specially designed approach still dominates in each time series analysis task such as classification, anomaly detection, forecasting, and few-shot learning. The main challenge that blocks the development of pre-trained model for time series analysis is the lack of a large amount of data for training. In this work, we address this challenge by leveraging language or CV models, pre-trained from billions of tokens, for time series analysis. Specifically, we refrain from altering the self-attention and feedforward layers of the residual blocks in the pre-trained language or image model. This model, known as the Frozen Pretrained Transformer (FPT), is evaluated through fine-tuning on all major types of tasks involving time series. Our results demonstrate that pre-trained models on natural language or images can lead to a comparable or state-of-the-art performance in all main time series analysis tasks, as illustrated in Figure 1. We also found both theoretically and empirically that the self-attention module behaviors similarly to principle component analysis (PCA), an observation that helps explains how transformer bridges the domain gap and a crucial step towards understanding the universality of a pre-trained transformer.The code is publicly available at https://github.com/DAMO-DI-ML/One_Fits_All.

==> sections/1_1_explaination_Jin.tex <==
\section{Analysis for Maximum Entropy Model for N-gram Estimation}
\def \y {\mathbf{y}}
\def \E {\mathrm{E}}
\def \x {\mathbf{x}}
\def \g {\mathbf{g}}
\def \L {\mathcal{L}}
\def \D {\mathcal{D}}
\def \z {\mathbf{z}}
\def \u {\mathbf{u}}
\def \H {\mathcal{H}}
\def \w {\mathbf{w}}
\def \R {\mathbb{R}}
\def \S {\mathcal{S}}
\def \regret {\mbox{regret}}
\def \Uh {\widehat{U}}
\def \Q {\mathcal{Q}}
\def \W {\mathcal{W}}
\def \N {\mathcal{N}}
\def \A {\mathcal{A}}
\def \q {\mathbf{q}}
\def \v {\mathbf{v}}
\def \M {\mathcal{M}}
\def \c {\mathbf{c}}
\def \ph {\widehat{p}}
\def \d {\mathbf{d}}
\def \p {\mathbf{p}}
\def \q {\mathbf{q}}
\def \db {\bar{\d}}
\def \dbb {\bar{d}}
\def \I {\mathcal{I}}
\def \f {\mathbf{f}}
\def \a {\mathbf{a}}
\def \b {\mathbf{b}}
\def \ft {\widetilde{\f}}
\def \bt {\widetilde{\b}}
\def \h {\mathbf{h}}
\def \B {\mathbf{B}}
\def \bts {\widetilde{b}}
\def \fts {\widetilde{f}}
\def \Gh {\widehat{G}}
\def \bh {\widehat{b}}
\def \fh {\widehat{f}}
\def \vb {\bar{v}}
\def \zt {\widetilde{\z}}
\def \zts {\widetilde{z}}
\def \s {\mathbf{s}}
\def \gh {\widehat{\g}}
\def \vh {\widehat{\v}}
\def \Sh {\widehat{S}}
\def \rhoh {\widehat{\rho}}
\def \hh {\widehat{\h}}
\def \C {\mathcal{C}}
\def \V {\mathcal{V}}
\def \t {\mathbf{t}}
\def \xh {\widehat{\x}}
\def \Ut {\widetilde{U}}
\def \wt {\widetilde{\w}}
\def \Th {\widehat{T}}
\def \Ot {\tilde{\mathcal{O}}}
\def \X {\mathcal{X}}
\def \nb {\widehat{\nabla}}
\def \K {\mathcal{K}}
\def \P {\mathbb{P}}
\def \T {\mathcal{T}}
\def \F {\mathcal{F}}
\def \ft{\widetilde{f}}
\def \xt {\widetilde{x}}
\def \Rt {\mathcal{R}}
\def \V {\mathcal{V}}
\def \Rb {\bar{\Rt}}
\def \wb {\bar{\w}}
\def \fh {\widehat{f}}
\def \wh {\widehat{\w}}
\def \lh {\widehat{\lambda}}
\def \e {\mathbf{e}}
\def \B {\mathcal{B}}
\def \xt {\widetilde{\x}}
\def \P {\mathcal{P}}
\def \vb {\bar{v}}
\def \ub {\bar{u}}
\def \Rt {\mathcal{R}}
\def \wh {\widehat{w}}
\def \Lh {\widehat{\L}}
\def \rh {\widehat{r}}
\def \G {\mathcal{G}}
\def \qh {\widehat{q}}
\def \Qh {\widehat{Q}}
\def \Gh {\widehat{G}}
\def \Ph {\widehat{P}}
\def \U {\mathcal{U}}
\textcolor{red}{Explaination from Dr Jin}

In this draft, we plan to show that for sequential data following power law, there is a potential universal solution to the final estimation of n-gram probabilities. For simplicity, we assume that $n$ is so large that we are unable to observe any occurrence of $n$-gram from data, and we only observe the occurrence of $n'$-grams with $n' < n$. We denote by $s^n_i$ the $i$th unique $n$-gram, and by the notation $s^{n'}_j \in s^n_i$ if $n'$-gram $s^{n'}_i$ appears in $s^n_i$, the $i$th $n$-gram. Let $m_n$ be the number of unique $n$-grams. According to the maximum entropy model, our estimation of n-gram probabilities can be cast into the following optimization problem:
\begin{equation}
\begin{split}
    \min\quad\sum_{i=1}^{m_n} &p(s^n_i)\log p(s^n_i) \\
    \textrm{s.t.} \sum_{i: s^{n'}_j \in s^n_i} &p(s^n_i) = \ph(s^{n'}_j), j\in [m_{n'}], n' \in [n-1] \\
    \sum_{i}&p(s_i^n) = 1
    \end{split}
\end{equation}
where $\ph(s^{n'}_j)$ represents the probability of observing pattern $s^{n'}_j$ from the data. 
For each constraint for $\ph(s_j^{n'})$, we introduce a Lagrangian dual variable $\lambda_{j}^{n'}$, and rewrite the optimization problem as follows
\begin{equation}
\min_{\lambda} \quad \log\left(\sum_{i=1}^{m_n} \exp\left(\sum_{(n',j): s^{n'}_j \in s^n_i} \lambda_j^{n'}\right)\right) - \sum_{n'=1}^{n-1}\sum_{j=1}^{m_{n'}} \lambda_{j}^{n'} \ph(s^{n'}_j)
\end{equation}
where n-gram probability $p(s^n_j)$ is given as
\begin{equation}
\begin{split}
p(s^n_j) = \frac{1}{Z(\lambda)}\exp\left(\sum_{(n',j):s_j^{n'} \in s_i^n} \lambda^{n'}_j\right) \\
\quad Z(\lambda) = \sum_{i=1}^{m_n} \exp\left(\sum_{(n',j):s_j^{n'} \in s_i^n} \lambda^{n'}_j\right)
\end{split}
\end{equation}
% {\color{blue}
% \begin{align}
%     \min_{p}\max_{\lambda}\quad\sum_{i=1}^{m_n} &p(s^n_i)\log p(s^n_i) + \sum_{jn'}\lambda_{j}^{n'} \left(\sum_{i: s^{n'}_j \in s^n_i} p(s^n_i) -\ph(s^{n'}_j)\right) + \lambda_0\left(\sum_{i} p(s_i^n)-1\right)\notag
%     % \textrm{s.t.} \sum_{i: s^{n'}_j \in s^n_i} &p(s^n_i) = \ph(s^{n'}_j), j\in [m_{n'}], n' \in [n-1]
% \end{align}


% \begin{align}
%     \max_{\lambda}\min_{p}\quad\sum_{i=1}^{m_n} &p(s^n_i)\left(\log p(s^n_i) + \sum_{s^{n'}_j \in s^n_i}\lambda_{j}^{n'} \right)-\sum_{jn'}\lambda_{j}^{n'}\ph(s^{n'}_j)+ \lambda_0\left(\sum_{i} p(s_i^n)-1\right)\notag
%     % \textrm{s.t.} \sum_{i: s^{n'}_j \in s^n_i} &p(s^n_i) = \ph(s^{n'}_j), j\in [m_{n'}], n' \in [n-1]
% \end{align}

% \begin{align}
%     &\log p(s^n_i) + \sum_{s^{n'}_j \in s^n_i}\lambda_{j}^{n'}  + p(s^n_i)\cdot\frac{1}{p(s^n_i)} + \lambda_0= 0\notag\\
%     &p(s^n_i) = \exp\left(-1-\lambda_0-\sum_{s^{n'}_j \in s^n_i}\lambda_{j}^{n'}\right)\notag\\
%     &\sum_{i}p(s^n_i) = \exp\left(-1-\lambda_0\right)\sum_{i}\exp\left(-\sum_{s^{n'}_j \in s^n_i}{\lambda}_{j}^{n'}\right) = 1\notag\\
%      &p(s^n_i) = \frac{1}{\sum_{i}\exp\left(\sum_{s^{n'}_j \in s^n_i}{\lambda}_{j}^{n'}\right)}\exp\left(-\sum_{s^{n'}_j \in s^n_i}{\lambda}_{j}^{n'}\right)\notag\\
%     &p(s^n_i) = \frac{1}{Z(\lambda)}\exp\left(-\sum_{s^{n'}_j \in s^n_i}{\lambda}_{j}^{n'}\right)\notag\\
%     %  &p(s^n_i) = \exp\left(\sum_{s^{n'}_j \in s^n_i}\lambda_{j}^{n'}\right)\notag\\
%     % &\sum_{i}p(s^n_i) = \sum_{i}\exp\left(-\frac{1+\lambda_0}{\sum_{s^{n'}_j \in s^n_i}\lambda_{j}^{n'}}\right) = 1\notag\\
%     % \textrm{s.t.} \sum_{i: s^{n'}_j \in s^n_i} &p(s^n_i) = \ph(s^{n'}_j), j\in [m_{n'}], n' \in [n-1]
% \end{align}
% \begin{align}
%  \max_{\lambda}\min_{p}\quad- &\frac{\log Z(\lambda)}{Z(\lambda)}\sum_{i=1}^{m_n}\exp\left(-\sum_{s^{n'}_j \in s^n_i}\tilde{\lambda}_{j}^{n'}\right)-\sum_{jn'}\lambda_{j}^{n'}\ph(s^{n'}_j)\notag\\
%   \max_{\lambda}\min_{p}\quad- &\log Z(\lambda)-\sum_{jn'}\lambda_{j}^{n'}\ph(s^{n'}_j)\notag
% \end{align}
% }
In the case that all n-grams follows power law, for each $n' \in [n-1]$, we divide $n'$-gram into two groups: the group $\V_{n'}$ includes the high frequency $n'$-gram and the group $\U_{n'}$ including the low frequency of $n'$-gram. For simplicity, we assume that the probability for all the high frequency $n'$-grams are roughly $\alpha_{n'} \in [0, 1]$ and the probability for all the low frequency $n'$-grams are roughly $\beta_{n'} \in [0, 1]$. Using these notations, we have the optimization problem simplified as
\begin{equation}
\resizebox{1.0\hsize}{!}{$
\begin{split}
\min_{\lambda}\quad\log\left(\sum_{i=1}^{m_n} \exp\left(\sum_{n'=1}^{n-1}\sum_{j: s^{n'}_j \in s^n_i} \lambda_a^{n'}I(s_j^{n'} \in \V_{n'}) + \lambda_b^{n'} I(s_j^{n'} \in \U_{n'})\right)\right) \\
- \sum_{n'=1}^{n-1}\lambda_a^{n'} g_{n'} + \lambda_b^{n'} h_{n'}
\end{split}
$}
\end{equation}
where
\begin{equation}
g_{n'} = \sum_{s^{n'}_j \in \V_{n'}} \ph(s^{n'}_j) \\
\quad h_{n'} = \sum_{s^{n'}_j \in \U_{n'}} \ph(s^{n'}_j)
\end{equation}
Note that in the above, by assuming that all the patterns in $\V_{n'}$ and $\U_{n'}$ share similar appearance frequency, we simplify the optimization problem by only introducing two dual variables for each $n'$-gram, i.e. $\lambda_a^{n'}$ for high-frequency patterns and $\lambda_b^{n'}$ for low-frequency patterns. Furthermore, let $q^{n'}_a$ be the probability to observe a high frequency $n'$-gram appearing in any $n$-gram, and $q^{n'}_b$ be the probability to observe a low frequency $n'$-gram appearing in any $n$-gram, we have
\begin{equation}
\resizebox{1.0\hsize}{!}{$
\begin{split}
&  & \sum_{i=1}^{m_n} \exp\left(\sum_{n'=1}^{n-1}\sum_{j: s^{n'}_j \in s^n_i} \lambda_a^{n'}I(s_j^{n'} \in \V_{n'}) + \lambda_b^{n'} I(s_j^{n'} \in \U_{n'})\right) \\
& = & m_n\prod_{n'=1}^{n-1}\left(1 + q_a^{n'}\exp(\lambda_a^{n'})\right)\left(1 + q_b^{n'}\exp(\lambda_b^{n'})\right) + \tilde{O}\left(\sqrt{m_n}\right)  
\end{split}
$}
\end{equation}

By skipping the term $O(\sqrt{m_n})$, we further simplify the optimization as
\begin{equation}
\resizebox{1.0\hsize}{!}{$
\begin{split}
\min_{\lambda} \quad \sum_{n'=1}^{n-1}\log\left(1 
+ q_a^{n'} \exp(\lambda_a^{n'})\right) + \log\left(1 + q_b^{n'}\exp(\lambda_b^{n'}\right) \\
- \lambda_{a}^{n'} g_{n'} - \lambda_b^{n'} h_{n'}
\end{split}
$}
\end{equation}
or
\begin{equation}
\begin{split}
\lambda_{n'}^a = \min_{\lambda} \log\left(1 + q_a^{n'}\exp(\lambda)\right) - \lambda g_n' \\
\quad \lambda_{n'}^b = \min_{\lambda}\log\left(1 + q_b^{n'}\exp(\lambda)\right) - \lambda h_n', 
\end{split}
\end{equation}
As illustrated by the above analysis, dual variables $\lambda_a^{n'}$ and $\lambda_b^{n'}$ will only depend on statistics $q_a^{n'}$, $q_b^{n'}$, $g_{n'}$ and $h_{n'}$. They are quite independent of detailed statistics $\ph(s^{n'}_j)$ and how each $n'$-gram appears in different $n$-gram. Thus, this simple analysis does indicate, to some degree, that the solution obtained from the maximum entropy model can be quite universal, as long as $n$-grams follow skewed distributions like power law. 


%% May be uesful
Transformer models can universally approximate arbitrary continuous sequence-to-sequence functions on a compact domain~\cite{Yun2020Are}



==> tables/tab_100_rebuttal.tex <==
\begin{table}
\caption{Results on full data. \textbf{Black}: best, {\color{red} \textbf{Red}}: second best.}
\label{tab:100_percent_ett}
\vskip 0.15in
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{c|c|cccccccccccccc}
\hline

\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{GPT2(6)}&\multicolumn{2}{c|}{GPT2(0)}&\multicolumn{2}{c|}{DLinear}&\multicolumn{2}{c|}{PatchTST}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c}{Informer}\\

\hline

\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE\\
\hline

\multirow{4}{*}{\rotatebox{90}{$ECL$}}
& 96  & 0.139 & 0.238 & \color{red}\textbf{0.138} & 0.234 & 0.140 & 0.237 & \textbf{0.129} & \textbf{0.222} & 0.186 & 0.302 & 0.196 & 0.313 & 0.304 & 0.393\\
& 192 & \color{red}\textbf{0.153} & 0.251 & \textbf{0.152} & 0.247 & \color{red}\textbf{0.153} & 0.249 & 0.157 & \textbf{0.240} &  0.197& 0.311& 0.211& 0.324& 0.327& 0.417\\
& 336 & 0.169 & 0.266 & \color{red}\textbf{0.168} & 0.263 & 0.169 & 0.267 & \textbf{0.163} & \textbf{0.259} &0.213 &0.328 &0.214& 0.327& 0.333& 0.422\\
& 720 & 0.206 & 0.297 & 0.207 & 0.295 & \color{red}\textbf{0.203} & 0.301 & \textbf{0.197} & \textbf{0.290} & 0.233& 0.344& 0.236& 0.342&0.351&0.427\\
\hline

\multirow{4}{*}{\rotatebox{90}{$Traffic$}}
& 96  & \color{red}\textbf{0.388} & 0.282 & 0.390 & \color{red}\textbf{0.272} & 0.410 & 0.282 & \textbf{0.360} & \textbf{0.249} & 0.576 &0.359 &0.597& 0.371& 0.733& 0.410\\
& 192 & 0.407 & 0.290 & \color{red}\textbf{0.403} & \color{red}\textbf{0.276} & 0.423 & 0.287 & \textbf{0.379} & \textbf{0.256} & 0.610 &0.380 &0.607& 0.382& 0.777& 0.435\\
& 336 & \color{red}\textbf{0.412} & 0.294 & 0.413 & \color{red}\textbf{0.280} & 0.436 & 0.296 & \textbf{0.392} & \textbf{0.264} & 0.608 &0.375 &0.623& 0.387& 0.776& 0.434 \\
& 720 & 0.450 & 0.312 & \color{red}\textbf{0.447} & \color{red}\textbf{0.298} & 0.466 & 0.315 & \textbf{0.432} & \textbf{0.286} & 0.621 &0.375& 0.639& 0.395& 0.827& 0.466\\

\hline
\hline
\end{tabular}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/tab_10_rebuttal.tex <==
\begin{table}
\caption{Few-shot learning results on 10\% data.}
\label{tab:10_percent_ett}
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{c|c|cccccccccccc}
\hline

\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{GPT2(6)}&\multicolumn{2}{c|}{GPT2(0)}&\multicolumn{2}{c|}{DLinear}&\multicolumn{2}{c|}{PatchTST}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c}{Autoformer}\\

\hline

\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\hline

\multirow{4}{*}{\rotatebox{90}{$ECL$}}
& 96  & \textbf{0.139} & \textbf{0.237} & 0.142 & 0.240 & 0.150 & 0.253 & 0.140 & 0.238 & 0.231 & 0.323 & 0.261 & 0.348 \\
& 192 & \textbf{0.156} & \textbf{0.252} & 0.158 & 0.254 & 0.164 & 0.264 & 0.160 & 0.255 & 0.261 & 0.356 & 0.338 & 0.406 \\
& 336 & \textbf{0.175} & \textbf{0.270} & \textbf{0.175} & 0.271 & 0.181 & 0.282 & 0.180 & 0.276 & 0.360 & 0.445 & 0.410 & 0.474 \\
& 720 & 0.233 & 0.317 & 0.230 & \textbf{0.315} & \textbf{0.223} & 0.321 & 0.241 & 0.323 & 0.530 & 0.585 & 0.715 & 0.685 \\
\hline

\multirow{4}{*}{\rotatebox{90}{$Traffic$}}
& 96  & 0.414 & 0.297 & 0.478 & 0.368 & 0.419 & 0.298 & \textbf{0.403} & \textbf{0.289} & 0.639 & 0.400 & 0.672 & 0.405 \\
& 192 & 0.426 & 0.301 & 0.481 & 0.363 & 0.434 & 0.305 & \textbf{0.415} & \textbf{0.296} & 0.637 & 0.416 & 0.727 & 0.424 \\
& 336 & 0.434 & \textbf{0.303} & 0.488 & 0.365 & 0.449 & 0.313 & \textbf{0.426} & 0.304 & 0.655 & 0.427 & 0.749 & 0.454 \\
& 720 & 0.487 & 0.337 & 0.537 & 0.386 & 0.484 & 0.336 & \textbf{0.474} & \textbf{0.331} & 0.722 & 0.456 & 0.847 & 0.499 \\

\hline
\hline

\end{tabular}
}
\end{small}
\end{center}
\end{table}

==> tables/tab_5_rebuttal.tex <==
\begin{table}
\caption{Few-shot learning results on 5\% data.}
\label{tab:5_percent_ett}
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{c|c|cccccccccccc}
\hline

\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{GPT2(6)}&\multicolumn{2}{c|}{GPT2(0)}&\multicolumn{2}{c|}{DLinear}&\multicolumn{2}{c|}{PatchTST}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c}{Autoformer}\\

\hline

\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\hline

\multirow{4}{*}{\rotatebox{90}{$ECL$}}
& 96  & \textbf{0.143} & \textbf{0.241} & 0.147 & 0.246 & 0.150 & 0.251 & 0.145 & 0.244 & 0.235 & 0.322 & 0.297 & 0.367 \\
& 192 & \textbf{0.159} & \textbf{0.255} & 0.163 & 0.260 & 0.163 & 0.263 & 0.163 & 0.260 & 0.247 & 0.341 & 0.308 & 0.375 \\
& 336 & \textbf{0.179} & \textbf{0.274} & 0.182 & 0.278 & 0.175 & 0.278 & 0.183 & 0.281 & 0.267 & 0.356 & 0.354 & 0.411 \\
& 720 & 0.233 & 0.323 & 0.239 & 0.329 & \textbf{0.219} & \textbf{0.311} & 0.233 & 0.323 & 0.318 & 0.394 & 0.426 & 0.466 \\
\hline

\multirow{4}{*}{\rotatebox{90}{$Traffic$}}
& 96  & 0.419 & 0.298 & 0.468 & 0.354 & 0.427 & 0.304 & \textbf{0.404} & \textbf{0.286} & 0.670 & 0.421 & 0.795 & 0.481 \\
& 192 & 0.434 & 0.305 & 0.479 & 0.352 & 0.447 & 0.315 & \textbf{0.412} & \textbf{0.294} & 0.653 & 0.405 & 0.837 & 0.503 \\
& 336 & 0.449 & 0.313 & 0.477 & 0.345 & 0.478 & 0.333 & \textbf{0.439} & \textbf{0.310} & 0.707 & 0.445 & 0.867 & 0.523 \\
& 720 & - & - & - & - & - & - & - & - & - & - & - & - \\
\hline
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table}

==> tables/tab_a_random_freeze.tex <==
\begin{table}
\caption{Ablation study on setting of "pretrain" and "freeze" on 5\% ETTh2.}
\begin{center}
\begin{tabular}{c|c|cccccccc}
\hline

\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{GPT2-FPT}&\multicolumn{2}{c|}{No Freeze}&\multicolumn{2}{c|}{No Pretrain}&\multicolumn{2}{c|}{No Pretrain + Freeze}\\

\hline

\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE\\
\hline
\multirow{2}{*}{\rotatebox{90}{\tiny $ETTh2$}}
& 96  & 0.376 & 0.421& 0.440 & 0.449& 0.465 & 0.457&0.540 & 0.497 \\
& 192 & 0.418 & 0.441& 0.503 & 0.478& 0.614 & 0.536&0.721 & 0.580 \\
\hline
\hline
\end{tabular}
\end{center}
\end{table}

==> tables/tab_ett_100percent_trans_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\setlength\tabcolsep{3pt} 
\centering
\begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Full results on full data. We use prediction length $O \in \{96, 192, 336, 720\}$ for ILI and $O \in \{24, 36, 48, 60\}$ for others. A lower MSE indicates better performance. \textbf{Black}: best, {\color{red} \textbf{Red}}: second best.}
\vskip 0.05in
\scalebox{0.65}{
\begin{tabular}{c|c|cccc|cccc|cccc|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Metric} &\multicolumn{4}{c|}{Weather}&\multicolumn{4}{c|}{ETTh1}&\multicolumn{4}{c|}{ETTh2}&\multicolumn{4}{c|}{ETTm1}&\multicolumn{4}{c|}{ETTm2}&\multicolumn{4}{c}{ILI}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
& &96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720
& 96 & 192 & 336 & 720
& 96 & 192 & 336 & 720& 24 & 36 & 48 & 60\\
\midrule
\multirow{2}{*}{GPT2-backbone(6 Layers)} & MSE & \color{red}\textbf{0.162} & \color{red}\textbf{0.204} & \color{red}\textbf{0.254} &\color{red}\textbf{0.326} & 0.376 & 0.416 & 0.442 & \textbf{0.447} & \color{red}\textbf{0.285} & \color{red}\textbf{0.354} & \color{red}\textbf{0.373} & \color{red}\textbf{0.406} & \color{red}\textbf{0.292} & \textbf{0.332} & \textbf{0.366} & \color{red}\textbf{0.417} & \color{red}\textbf{0.173} & \color{red}\textbf{0.229} & \color{red}\textbf{0.286} & \color{red}\textbf{0.378} & \color{red}\textbf{2.063} & \color{red}\textbf{1.868} & \color{red}\textbf{1.790} & 1.979 \\
& MAE &\color{red}\textbf{0.212} &\color{red}\textbf{0.248} &\color{red}\textbf{0.286} &\color{red}\textbf{0.337} &\textbf{0.397} & \color{red}\textbf{0.418} &\textbf{0.433} &\textbf{0.456} &\color{red}\textbf{0.342} &\color{red}\textbf{0.389} &\color{red}\textbf{0.407} &\color{red}\textbf{0.441} &0.346 &0.372 &0.394 &\color{red}\textbf{0.421} &\color{red}\textbf{0.262} &\color{red}\textbf{0.301} &\color{red}\textbf{0.341} &\color{red}\textbf{0.401} & \color{red}\textbf{0.881} & \color{red}\textbf{0.892} & \color{red}\textbf{0.884} & \color{red}\textbf{0.957} \\\midrule

\multirow{2}{*}{GPT2-backbone(0 Layer)} & MSE & 0.181 &0.222 &0.270& 0.338 &0.422 &0.466 &0.488 &0.485 &0.318 &0.383 &0.406 &0.420 &0.330 &0.371 &0.398 &0.454 &0.192 &0.245 &0.302 &0.399 & 2.723 & 2.027 & 2.206 &  \color{red}\textbf{1.976} \\
& MAE &0.232 &0.266 &0.299 &0.345 &0.428&0.450 &0.464 & 0.478& 0.368& 0.407&0.427 &0.446 &0.372 &0.394 &0.409 &0.440 &0.281 &0.317 &0.352 &0.408 & 1.099 & 0.966 & 1.022 & 0.983 \\\midrule

\multirow{2}{*}{DLinear\cite{dlinear}} & MSE &0.176 &0.220 &0.265 &0.323 &\color{red}\textbf{0.375} &\textbf{0.405} &\color{red}\textbf{0.439} &0.472 &0.289 &0.383 &0.448 &0.605 &0.299 &0.335 &0.369 &0.425 &0.167 &0.224 &0.281 &0.397 &2.215 &1.963 &2.130 &2.368  \\
& MAE &0.237 &0.282 &0.319 &0.362 &\color{red}\textbf{0.399} &\textbf{0.416} &0.443 &0.490 &0.353 &0.418 &0.465 &0.551 &\color{red}\textbf{0.343} &\textbf{0.365} &\textbf{0.386} &\color{red}\textbf{0.421} &0.269 &0.303 &0.342 & 0.421 &1.081 &0.963 &1.024 &1.096 \\\midrule

\multirow{2}{*}{PatchTST\cite{Patchformer}} & MSE &\textbf{0.149} & \textbf{0.194} &\textbf{0.245} &\textbf{0.314} &\textbf{0.370} &0.413 &\textbf{0.422} &\textbf{0.447} &\textbf{0.274} &\textbf{0.339} &\textbf{0.329} &\textbf{0.379} &\textbf{0.290} &\textbf{0.332} &\textbf{0.366} &\textbf{0.416} &\textbf{0.165} &\textbf{0.220} &\textbf{0.274} &\textbf{0.362} &\textbf{1.319} &\textbf{1.430} &\textbf{1.553} &\textbf{1.470}  \\
& MAE &\textbf{0.198} &\textbf{0.241} &\textbf{0.282} &\textbf{0.334} &\color{red}\textbf{0.399} &0.421 &\color{red}\textbf{0.436} &\color{red}\textbf{0.466} &\textbf{0.336} &\textbf{0.379} &\textbf{0.380} &\textbf{0.422} &\textbf{0.342} &\color{red}\textbf{0.369} &\color{red}\textbf{0.392} &\textbf{0.420} &\textbf{0.255} &\textbf{0.292} &\textbf{0.329} &\textbf{0.385} &\textbf{0.754} &\textbf{0.834} &\textbf{0.815} &\textbf{0.788}  \\\midrule


\multirow{2}{*}{FEDformer\cite{zhou2022fedformer}} & MSE &0.217&0.276&0.339&0.403&0.376&0.420&0.459&0.506&0.346&0.429&0.496&0.463&0.379&0.426&0.445&0.543&0.203&0.269&0.325&0.421&3.228&2.679&2.622&2.857\\
& MAE  &0.296&0.336&0.380&0.428&0.419&0.448&0.465&0.507&0.388&0.439&0.487&0.474&0.419&0.441&0.459&0.490&0.287&0.328&0.366&0.415&1.260&1.080&1.078&1.157\\\midrule

\multirow{2}{*}{Autoformer\cite{wu2021autoformer}} & MSE&0.266&0.307&0.359&0.419&0.449&0.500&0.521&0.514&0.358&0.456&0.482&0.515&0.505&0.553&0.621&0.671&0.255&0.281&0.339&0.433&3.483&3.103&2.669&2.770\\
& MAE &0.336&0.367&0.395&0.428&0.459&0.482&0.496&0.512&0.397&0.452&0.486&0.511&0.475&0.496&0.537&0.561&0.336&0.340&0.372&0.432&1.287&1.148&1.085&1.125 \\\midrule

\multirow{2}{*}{Informer\cite{zhou2021informer}} & MSE&0.300&0.598&0.578&1.059&0.865&1.008&1.107&1.181&3.755&5.602&4.721&3.647&0.672&0.795&1.212&1.166&0.365&0.533&1.363&3.379&5.764&4.755&4.763&5.264\\
& MAE &0.384&0.544&0.523&0.741&0.713&0.792&0.809&0.865&1.525&1.931&1.835&1.625&0.571&0.669&0.871&0.823&0.453&0.563&0.887&1.338&1.677&1.467&1.469&1.564 \\


\bottomrule
\end{tabular}
\label{tab:100_percent_ett}
}
% \end{adjustwidth}
\end{small}
\vskip -0.1in
\end{table*}
%}

==> tables/tab_ett_10percent_trans.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[!h]
\setlength\tabcolsep{3pt} 
\centering
\begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Few-shot learning results on 10\% data. We use prediction length $O \in \{96, 192, 336, 720\}$ for ILI and $O \in \{24, 36, 48, 60\}$ for others. A lower MSE indicates better performance, and the best results are highlighted in bold. '-' means that 10\% time series is not sufficient to constitute a training set.}
\vskip 0.05in
\scalebox{0.61}{
\begin{tabular}{c|c|cccc|cccc|cccc|cccc|cccc|cccc|c}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Metric} &\multicolumn{4}{c|}{Weather}&\multicolumn{4}{c|}{ETTh1}&\multicolumn{4}{c|}{ETTh2}&\multicolumn{4}{c|}{ETTm1}&\multicolumn{4}{c|}{ETTm2}&\multicolumn{4}{c|}{ILI} & \multirow{2}{*}{Count}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
& &96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720
& 96 & 192 & 336 & 720
& 96 & 192 & 336 & 720& 24 & 36 & 48 & 60\\
\midrule
\multirow{2}{*}{GPT2-backbone(6 Layers)} & MSE & \textbf{0.163} & \textbf{0.210} & \textbf{0.256} & 0.321 & \textbf{0.458} & 0.570 & \textbf{0.608} & 0.725 & \textbf{0.331} & \textbf{0.402} & \textbf{0.406} & \textbf{0.449} & 0.390 & 0.429 & 0.469 & 0.569 & \textbf{0.188} & \textbf{0.251} & 0.307 & \textbf{0.426} & \textbf{3.022} & 3.854 & 4.603 & - & \textbf{13}\\
& MAE & \textbf{0.215} & \textbf{0.254} & \textbf{0.292} & \textbf{0.339} & \textbf{0.456} &  \textbf{0.516}& \textbf{0.535} & \textbf{0.591} & \textbf{0.374} & \textbf{0.411} & \textbf{0.433} & \textbf{0.464} & 0.404 & 0.423 & 0.439 & 0.498 & \textbf{0.269} & \textbf{0.309} & \textbf{0.346} & \textbf{0.417} & \textbf{1.247} & 1.453 & 1.571 & - & \textbf{17}\\\midrule

\multirow{2}{*}{GPT2-backbone(0 Layer)} & MSE & 0.190 & 0.243 & 0.270 & 0.348 & 0.601 & 0.709 & 0.801 & 1.385 & 0.539 & 0.675 & 0.718 & 0.732 & 0.610 & 0.666 & 0.895 & 0.916 & 0.283 & 0.353 & 0.420 & 0.553 & 3.521 & 3.446 & 4.435 & - & 0 \\
& MAE & 0.240 & 0.284 & 0.305 & 0.359 & 0.536 & 0.587 & 0.635 & 0.831 & 0.495 & 0.555 & 0.580 & 0.605 & 0.508 & 0.540 & 0.615 & 0.646 & 0.344 & 0.384 & 0.422 & 0.491 & 1.274 & 1.340 & 1.554 & - & 0\\\midrule

\multirow{2}{*}{DLinear\cite{dlinear}} & MSE & 0.171 & 0.215 & 0.258 & \textbf{0.320} & 0.492 & \textbf{0.565} & 0.721 & 0.986 & 0.357 & 0.569 & 0.671 & 0.824 & \textbf{0.352} & \textbf{0.382} & \textbf{0.419} & \textbf{0.490} & 0.213 & 0.278 & 0.338 & 0.436 & 3.969 & 3.700 & 3.980 & - & 6\\
& MAE & 0.224 & 0.263 & 0.299 & 0.346 & 0.495 & 0.538 & 0.622 & 0.743 & 0.411 & 0.519 & 0.572 & 0.648 & \textbf{0.392} & \textbf{0.412} & \textbf{0.434} & \textbf{0.477} & 0.303 & 0.345 & 0.385 & 0.440 & 1.536 & 1.467 & 1.485 & - & 4\\\midrule

\multirow{2}{*}{PatchTST\cite{Patchformer}} & MSE & 0.165 & 0.210 & 0.259 & 0.332 & 0.516 & 0.598 & 0.657 & 0.762 & 0.353 & 0.403 & 0.426 & 0.477 & 0.410 & 0.437 & 0.476 & 0.681 & 0.191 & 0.252 & \textbf{0.306} & 0.433 & 3.144 & \textbf{2.950} & \textbf{3.501} & - & 3\\
& MAE & 0.215 & 0.257 & 0.297 & 0.346 & 0.485 & 0.524 & 0.550 & 0.610 & 0.389 & 0.414 & 0.441 & 0.480 & 0.419 & 0.434 & 0.454 & 0.556 & 0.274 & 0.317 & 0.353 & 0.427 & 1.261 & \textbf{1.237} & \textbf{1.358} & - & 2\\\midrule


\multirow{2}{*}{FEDformer\cite{zhou2022fedformer}} & MSE &0.188&0.250&0.312&0.387&0.512&0.624&0.691&0.728&0.382&0.478&0.504&0.499&0.578&0.617&0.998&0.693&0.291&0.307&0.543&0.712&4.338&5.166&4.404&4.380&0\\
& MAE  &0.253&0.304&0.346&0.393&0.499&0.555&0.574&0.614&0.416&0.474&0.501&0.509&0.518&0.546&0.775&0.579&0.399&0.379&0.559&0.614&1.525&1.658&1.523&\textbf{1.498}&1\\\midrule

\multirow{2}{*}{Autoformer\cite{wu2021autoformer}} & MSE &0.221&0.270&0.320&0.390&0.613&0.722&0.750&\textbf{0.721}&0.413&0.474&0.547&0.516&0.774&0.754&0.869&0.810&0.352&0.694&2.408&1.913&3.733&4.342&4.267&\textbf{4.429}&2\\
& MAE  &0.297&0.322&0.351&0.396&0.552&0.598&0.619&0.616&0.451&0.477&0.543&0.523&0.614&0.592&0.677&0.630&0.454&0.691&1.407&1.166&1.380&1.507&1.493&1.527&0\\

\bottomrule
\end{tabular}
\label{tab:10_percent_ett}
}
% \end{adjustwidth}
\end{small}
\vskip -0.1in
\end{table*}
%}

==> tables/tab_ett_5percent_trans.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[t]
\setlength\tabcolsep{3pt} 
\centering
\begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Few-shot learning results on 5\% data. We use prediction length $O \in \{96, 192, 336, 720\}$ for ILI and $O \in \{24, 36, 48, 60\}$ for others. A lower MSE indicates better performance, and the best results are highlighted in bold. '-' means that 5\% time series is not sufficient to constitute a training set.}
\vskip 0.05in
\scalebox{0.65}{
\begin{tabular}{c|c|cccc|cccc|cccc|cccc|cccc|cccc|c}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Metric} &\multicolumn{4}{c|}{Weather}&\multicolumn{4}{c|}{ETTh1}&\multicolumn{4}{c|}{ETTh2}&\multicolumn{4}{c|}{ETTm1}&\multicolumn{4}{c|}{ETTm2}&\multicolumn{4}{c|}{ILI}&\multirow{2}{*}{Count}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
& &96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720
& 96 & 192 & 336 & 720
& 96 & 192 & 336 & 720& 24 & 36 & 48 & 60\\
\midrule
\multirow{2}{*}{GPT2-backbone(6 Layers)} & MSE & 0.175 & \textbf{0.227} & 0.286 & 0.366 & \textbf{0.543} & 0.748 & 0.754 & - & \textbf{0.376} & \textbf{0.418} & \textbf{0.408} & - & 0.386 & 0.440 & 0.485 & 0.557 & \textbf{0.199} & \textbf{0.256} & \textbf{0.318} & 0.460 & 4.225 & - & - & - & \textbf{8}\\
& MAE & \textbf{0.230} & \textbf{0.276} & 0.322 & \textbf{0.379} & 0.506 & 0.580 & 0.595 & - & \textbf{0.421} & \textbf{0.441} & \textbf{0.439} & - & 0.405 & 0.438 & 0.459 & 0.499 & \textbf{0.280} & \textbf{0.316} & \textbf{0.353} & 0.436 & 1.588 & - & - & - & \textbf{9}\\\midrule

\multirow{2}{*}{GPT2-backbone(0 Layer)} & MSE & 0.191 & 0.244 & 0.303 & 0.391 & 0.825 & 1.220 & 1.852 & - & 0.551 & 0.765 & 0.767 & - & 0.582 & 0.632 & 0.767 & 1.334 & 0.282 & 0.346 & 0.429 & 0.751 & 6.565 & - & - & - & 0\\
& MAE & 0.243 & 0.289 & 0.332 & 0.393 & 0.638 & 0.778 & 0.965 & - & 0.507 & 0.610 & 0.614 & - & 0.512 & 0.536 & 0.584 & 0.742 & 0.347 & 0.383 & 0.427 & 0.568 & 1.894 & - & - & - & 0\\\midrule

\multirow{2}{*}{DLinear\cite{dlinear}} & MSE & 0.184 & 0.228 & \textbf{0.279} & \textbf{0.364} & 0.547 & 0.720 & 0.984 & - & 0.442 & 0.617 & 1.424 & - & \textbf{0.332} & \textbf{0.358} & \textbf{0.402} & \textbf{0.511} & 0.236 & 0.306 & 0.380 & 0.674 & 4.803 & - & - & - & 6\\
& MAE & 0.242 & 0.283 & \textbf{0.322} & 0.388 & \textbf{0.503} & 0.604 & 0.727 & - & 0.456 & 0.542 & 0.849 & - & \textbf{0.374} & \textbf{0.390} & \textbf{0.416} & \textbf{0.489} & 0.326 & 0.373 & 0.423 & 0.583 & 1.657 & - & - & - & 6\\\midrule

\multirow{2}{*}{PatchTST\cite{Patchformer}} & MSE & \textbf{0.171} & 0.230 & 0.294 & 0.384 & 0.557 & 0.711 & 0.816 & - & 0.401 & 0.452 & 0.464 & - & 0.399 & 0.441 & 0.499 & 0.767 & 0.206 & 0.264 & 0.334 & \textbf{0.454} & \textbf{3.749} & - & - & - & 3\\
& MAE & 0.224 & 0.277 & 0.326 & 0.387 & 0.519 & 0.570 & 0.619 & - & 0.421 & 0.455 & 0.469 & - & 0.414 & 0.436 & 0.467 & 0.587 & 0.288 & 0.324 & 0.367 & \textbf{0.432} & \textbf{1.419} & - & - & - & 2\\\midrule


\multirow{2}{*}{FEDformer\cite{zhou2022fedformer}} & MSE &0.229&0.265&0.353&0.391&0.593&\textbf{0.652}&\textbf{0.731}&-&0.390&0.457&0.477&-&0.628&0.666&0.807&0.822&0.229&0.294&0.378&0.523&5.193&-&-&-&2\\
& MAE  &0.309&0.317&0.392&0.394&0.529&\textbf{0.563}&\textbf{0.594}&-&0.424&0.465&0.483&-&0.544&0.566&0.628&0.633&0.320&0.361&0.427&0.510&1.691&-&-&-&2\\\midrule

\multirow{2}{*}{Autoformer\cite{wu2021autoformer}} & MSE &0.227&0.278&0.351&0.387&0.681&0.725&0.761&-&0.428&0.496&0.486&-&0.726&0.750&0.851&0.857&0.232&0.291&0.478&0.553&5.404&-&-&-&0\\
& MAE  &0.299&0.333&0.393&0.389&0.570&0.602&0.624&-&0.468&0.504&0.496&-&0.578&0.591&0.659&0.655&0.322&0.357&0.517&0.538&1.756&-&-&-&0\\


\bottomrule
\end{tabular}
\label{tab:5_percent_ett}
}
% \end{adjustwidth}
\end{small}
\vskip -0.1in
\end{table*}
%}

==> tables/tab_ett_other_model.tex <==
\begin{table*}[h]
\caption{Results of frozen pretrained transformer variants.}
\vskip 0.15in
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{6 Layers}&\multicolumn{2}{c|}{BERT}&\multicolumn{2}{c|}{BEiT}&\multicolumn{2}{c|}{DLinear}&\multicolumn{2}{c|}{PatchTST}\\

\midrule

\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE & MSE  & MAE & MSE  & MAE \\
\midrule


\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
& 96 &&&&&&&&&&\\
& 192  &&&&&&&&&&\\
& 336  &&&&&&&&&&\\
& 720  &&&&&&&&&&\\
\midrule


\multirow{4}{*}{\rotatebox{90}{$ETTm2$}}
& 96 &&&&&&&&&&\\
& 192  &&&&&&&&&&\\
& 336  &&&&&&&&&&\\
& 720  &&&&&&&&&&\\

\bottomrule
\end{tabular}
}
\label{tab:ett_other_model}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/tab_monash_10percent.tex <==
\begin{table*}[h]
\caption{Results on 10\% Monash data (sMAPE).}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{c|ccc|ccc}
\toprule

Methods & 6 Layers & 0 Layer & DLinear & FULL DeepAR & FULL N-BEATS & FULL ARIMA \\

\midrule

M3 Yearly &  & & & 17.24 & 17.03 & 18.84 \\
M3 Quarterly & & & & 9.93 & 9.47 & 10.24 \\
M3 Monthly & & & & 15.74 & 14.67 & 14.24 \\
M3 Other & & & & 5.57 & 4.97 & 4.35 \\
\midrule

M4 Yearly & \textbf{14.85} & 14.99 & 16.77 & - & - & 16.03\\
M4 Quarterly & \textbf{10.88} & 11.11 & 18.77 & 10.64 & 10.46 & 10.52 \\
M4 Monthly & \textbf{13.67} & 13.87 & 55.33 & 14.29 & 13.40 & 13.08 \\
M4 Weekly & \textbf{7.09} & 8.30 & 7.79 & 7.93 & 6.81 & 7.94 \\
M4 Daily & \textbf{2.99} & \textbf{2.99} & 12.38 & 5.04 & 3.20 & 3.01\\
M4 Hourly & \textbf{14.11} & 19.12 & 20.43 & 15.07 & 15.75 & 35.99 \\
\midrule

Tourism Yearly & - & - & - & 34.09 & 30.27 & 33.44 \\
Tourism Quarterly & \textbf{18.34} & 20.10 & 41.07 & 15.29 & 14.45 & 16.58 \\
Tourism Monthly & \textbf{23.86} & 177.26 & 29.22 & 18.35 & 20.42 & 19.73 \\

\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/tab_monash_5percent.tex <==
\begin{table*}[h]
\caption{Results on 5\% Monash data (sMAPE).}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{c|ccc|ccc}
\toprule

Methods & 6 Layers & 0 Layer & DLinear & FULL DeepAR & FULL N-BEATS & FULL ARIMA \\

\midrule

M3 Yearly &  & & & 17.24 & 17.03 & 18.84 \\
M3 Quarterly & & & & 9.93 & 9.47 & 10.24 \\
M3 Monthly & & & & 15.74 & 14.67 & 14.24 \\
M3 Other & & & & 5.57 & 4.97 & 4.35 \\
\midrule

M4 Yearly & 15.08 & \textbf{14.99} & 46.64 & - & - & 16.03\\
M4 Quarterly & \textbf{11.07} & 11.35 & 27.16 & 10.64 & 10.46 & 10.52 \\
M4 Monthly & \textbf{14.08} & 14.85 & 56.21 & 14.29 & 13.40 & 13.08 \\
M4 Weekly & \textbf{7.86} & 21.61 & 8.13 & 7.93 & 6.81 & 7.94 \\
M4 Daily & \textbf{2.97} & 3.00 & 21.89 & 5.04 & 3.20 & 3.01\\
M4 Hourly & - & - & - & 15.07 & 15.75 & 35.99 \\
\midrule

Tourism Yearly & - & - & - & 34.09 & 30.27 & 33.44 \\
Tourism Quarterly & - & - & - & 15.29 & 14.45 & 16.58 \\
Tourism Monthly & - & - & - & 18.35 & 20.42 & 19.73 \\

\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
